Parametrized Asymmetric Neutral hydrogen Disk Integrated Spectrum Characterization (PANDISC) I: Introduction to A Physically Motivated H I Model

Modelling the integrated H I spectra of galaxies has been a difficult task due to their diverse shapes, but more dynamical information is waiting to be explored in Hi line profiles. Based on simple assumptions, we construct a physically motivated model for the integrated Hi spectra: Parametrized Asymmetric Neutral hydrogen Disk Integrated Spectrum Characterization (PANDISC). The model shows great flexibility in reproducing the diverse Hi profiles. We use Monte-Carlo Markov Chain (MCMC) for fitting the model to global H I profiles, producing statistically robust quantitative results. Comparing with several samples of H I data available in the literature , we find the model-fitted results agree with catalogued velocity widths (e.g., W50) down to the lowest S/N. The model is also shown to be useful for applications like the baryonic Tully-Fisher relation (BTFR) and profile-based sample control. By comparing v_r to v_flat , we uncover how the H I width is affected by the structure of the rotation curve, following a trend consistent with the difference in the BTFR slope. We also select a sample of spectra with broad wing-like features suggestive of a population of galaxies with unusual gas dynamics. The PANDISC model bears both promise and limitations for potential use beyond H I lines. Further application on the whole ALFALFA sample will enable us to perform large scale ensemble studies of the H I properties and dynamics in nearby galaxies.

==> combined_table_partial.tex <==
\begin{tabular}{ccccccccccccccc}
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) & (14) & (15)\\ 
Name & Alternative Name & Sample & Reference & $v_r$ & $k$ & $v_\sigma$ & $r$ & $v_g$ & $F$ & $v_c$ & $W50_\mathrm{model}$ & SRD & rms$_\mathrm{blank}$ & rms$_\mathrm{residual}$ \\
 &  &  &  & $\mathrm{km\,s^{-1}}$ &  & $\mathrm{km\,s^{-1}}$ &  & $\mathrm{km\,s^{-1}}$ & $\mathrm{Jy\,km\,s^{-1}}$ & $\mathrm{km\,s^{-1}}$ & $\mathrm{km\,s^{-1}}$ &  &  &  \\
\hline
AGC000027 & CGCG 408-020 & high S/N & a.100 & 99.93$^{+0.41} _{-0.41}$ & 0.024$^{+0.011} _{-0.011}$ & 13.15$^{+0.46} _{-0.44}$ & 0.919$^{+0.025} _{-0.025}$ & 58.56$^{+10.08} _{-10.09}$ & 13.69$^{+0.15} _{-0.14}$ & 3113.42$^{+0.36} _{-0.39}$ & 216.69$^{+1.12} _{-1.09}$ & 106.7 & 2.07 & 2.11 \\
AGC000075$^\star$$^\ddagger$ & NGC  14 & high S/N & a.100 & 45.84$^{+1.06} _{-1.38}$ & 0.557$^{+0.051} _{-0.072}$ & 17.53$^{+0.59} _{-0.56}$ & 0.741$^{+0.043} _{-0.062}$ & 20.82$^{+2.47} _{-2.0}$ & 18.06$^{+0.13} _{-0.13}$ & 868.95$^{+1.87} _{-2.03}$ & 104.82$^{+3.5} _{-4.02}$ & 164.5 & 2.55 & 2.8 \\
AGC000099 & M+201023 & high S/N & a.100 & 33.69$^{+0.42} _{-0.43}$ & 0.017$^{+0.014} _{-0.015}$ & 10.34$^{+0.48} _{-0.57}$ & 0.858$^{+0.093} _{-0.089}$ & 22.97$^{+4.37} _{-9.33}$ & 9.93$^{+0.12} _{-0.09}$ & 1740.0$^{+0.27} _{-0.27}$ & 78.8$^{+1.08} _{-0.98}$ & 117.3 & 2.18 & 2.63 \\
AGC000122$^\ddagger$ & CGCG 456-039 & high S/N & a.100 & 44.75$^{+0.31} _{-0.28}$ & 0.18$^{+0.023} _{-0.022}$ & 7.5$^{+0.36} _{-0.3}$ & 0.501$^{+0.046} _{-0.037}$ & 26.39$^{+1.23} _{-1.56}$ & 14.85$^{+0.13} _{-0.13}$ & 854.02$^{+0.3} _{-0.28}$ & 91.5$^{+1.48} _{-1.1}$ & 146.9 & 2.42 & 2.96 \\
AGC000156 & CGCG 433-041 & high S/N & a.100 & 57.31$^{+0.68} _{-0.78}$ & -0.17$^{+0.019} _{-0.02}$ & 12.57$^{+0.65} _{-0.63}$ & 0.74$^{+0.049} _{-0.057}$ & 24.77$^{+3.28} _{-2.99}$ & 13.19$^{+0.11} _{-0.12}$ & 1134.53$^{+0.47} _{-0.5}$ & 127.54$^{+1.2} _{-1.67}$ & 123.5 & 2.23 & 3.34 \\
AGC000191 & CGCG 434-001,UGC 191 & high S/N,SPARC & a.100 & 57.66$^{+0.28} _{-0.28}$ & -0.03$^{+0.011} _{-0.012}$ & 9.75$^{+0.35} _{-0.32}$ & 0.74$^{+0.032} _{-0.029}$ & 41.2$^{+2.3} _{-2.59}$ & 17.37$^{+0.16} _{-0.15}$ & 1144.03$^{+0.25} _{-0.25}$ & 125.25$^{+0.66} _{-0.65}$ & 138.7 & 2.58 & 3.0 \\
AGC000230 & NGC  99 & high S/N & a.100 & 58.44$^{+0.45} _{-0.45}$ & -0.063$^{+0.014} _{-0.014}$ & 16.13$^{+0.61} _{-0.69}$ & 0.929$^{+0.042} _{-0.051}$ & 82.34$^{+45.29} _{-17.94}$ & 13.48$^{+0.21} _{-0.2}$ & 5312.92$^{+0.48} _{-0.48}$ & 139.74$^{+1.77} _{-1.46}$ & 105.1 & 2.44 & 2.83 \\
AGC000231$^\ddagger$ & NGC 100 & high S/N,SPARC & a.100 & 94.77$^{+0.16} _{-0.17}$ & -0.087$^{+0.005} _{-0.005}$ & 10.97$^{+0.2} _{-0.2}$ & 0.712$^{+0.012} _{-0.012}$ & 54.47$^{+1.33} _{-1.34}$ & 44.85$^{+0.18} _{-0.18}$ & 842.35$^{+0.15} _{-0.16}$ & 198.43$^{+0.52} _{-0.49}$ & 280.1 & 2.66 & 5.97 \\
AGC000260$^\ddagger$ & CGCG 434-013 & high S/N & a.100 & 116.79$^{+0.28} _{-0.28}$ & -0.118$^{+0.006} _{-0.006}$ & 17.05$^{+0.35} _{-0.35}$ & 0.853$^{+0.017} _{-0.018}$ & 68.64$^{+4.63} _{-4.74}$ & 34.33$^{+0.18} _{-0.18}$ & 2133.87$^{+0.27} _{-0.28}$ & 253.11$^{+0.94} _{-0.87}$ & 226.8 & 2.25 & 3.47 \\
AGC000369 & NGC 173 & high S/N & a.100 & 140.48$^{+0.44} _{-0.46}$ & 0.001$^{+0.011} _{-0.011}$ & 13.9$^{+0.62} _{-0.57}$ & 0.859$^{+0.031} _{-0.029}$ & 92.74$^{+10.59} _{-13.04}$ & 21.7$^{+0.26} _{-0.25}$ & 4367.77$^{+0.42} _{-0.41}$ & 297.4$^{+1.39} _{-1.3}$ & 107.6 & 2.77 & 2.86 \\
AGC000477$^\ddagger$ & CGCG 458-004 & high S/N & a.100 & 110.4$^{+0.3} _{-0.3}$ & 0.042$^{+0.009} _{-0.009}$ & 12.36$^{+0.39} _{-0.39}$ & 0.714$^{+0.021} _{-0.019}$ & 68.39$^{+2.55} _{-2.91}$ & 27.4$^{+0.2} _{-0.18}$ & 2647.99$^{+0.29} _{-0.28}$ & 230.97$^{+0.89} _{-0.8}$ & 169.4 & 2.48 & 3.35 \\
AGC000499$^\mathsection$ & NGC 262 & high S/N & a.100 & 22.36$^{+0.31} _{-0.31}$ & 0.169$^{+0.026} _{-0.024}$ & 11.76$^{+0.57} _{-0.57}$ & 0.568$^{+0.076} _{-0.079}$ & 31.41$^{+2.31} _{-1.71}$ & 14.37$^{+0.11} _{-0.12}$ & 4541.76$^{+0.34} _{-0.33}$ & 62.48$^{+0.74} _{-0.71}$ & 176.2 & 2.13 & 3.03 \\
AGC000521$^\ddagger$ & CGCG 435-014 & high S/N & a.100 & 56.03$^{+1.82} _{-2.06}$ & 0.077$^{+0.031} _{-0.034}$ & 14.32$^{+1.54} _{-1.29}$ & 0.625$^{+0.06} _{-0.06}$ & 19.61$^{+1.9} _{-1.84}$ & 13.95$^{+0.13} _{-0.13}$ & 663.96$^{+0.75} _{-0.74}$ & 126.43$^{+1.59} _{-1.89}$ & 131.2 & 2.31 & 3.71 \\
AGC000634 & CGCG 410-023,UGC 634 & high S/N,SPARC & a.100 & 59.31$^{+0.51} _{-0.53}$ & 0.118$^{+0.012} _{-0.012}$ & 14.86$^{+0.45} _{-0.44}$ & 0.934$^{+0.029} _{-0.035}$ & 30.12$^{+6.37} _{-7.82}$ & 14.89$^{+0.14} _{-0.13}$ & 2213.76$^{+0.4} _{-0.42}$ & 137.13$^{+0.96} _{-1.01}$ & 124.9 & 2.37 & 2.88 \\
AGC000668$^\mathsection$ & IC 1613 & high S/N & a.100 & 6.88$^{+0.01} _{-0.01}$ & -0.158$^{+0.002} _{-0.002}$ & 6.52$^{+0.01} _{-0.01}$ & 0.578$^{+0.004} _{-0.004}$ & 14.38$^{+0.06} _{-0.06}$ & 337.46$^{+0.19} _{-0.19}$ & -232.15$^{+0.01} _{-0.01}$ & 23.92$^{+0.02} _{-0.02}$ & 2798.4 & 5.17 & 20.09 \\
AGC000685$^\ast$ & CGCG 458-020 & high S/N & a.100 & 29.16$^{+0.27} _{-0.24}$ & 0.122$^{+0.014} _{-0.014}$ & 12.33$^{+0.36} _{-0.48}$ & 0.937$^{+0.041} _{-0.073}$ & 41.36$^{+44.9} _{-10.69}$ & 13.2$^{+0.16} _{-0.14}$ & 156.75$^{+0.28} _{-0.29}$ & 73.22$^{+0.97} _{-0.74}$ & 146.0 & 2.36 & 4.85 \\
AGC000763$^\ast$ & NGC 428 & high S/N & a.100 & 68.43$^{+0.18} _{-0.18}$ & -0.006$^{+0.004} _{-0.004}$ & 15.79$^{+0.23} _{-0.22}$ & 0.876$^{+0.015} _{-0.014}$ & 57.27$^{+2.38} _{-2.61}$ & 67.69$^{+0.24} _{-0.22}$ & 1153.15$^{+0.14} _{-0.14}$ & 156.69$^{+0.34} _{-0.33}$ & 398.3 & 3.12 & 14.79 \\
AGC000891$^\ast$ & CGCG 436-033,UGC 891 & high S/N,SPARC & a.100 & 51.12$^{+0.34} _{-0.36}$ & -0.068$^{+0.019} _{-0.019}$ & 9.15$^{+0.44} _{-0.41}$ & 0.539$^{+0.037} _{-0.032}$ & 30.73$^{+1.21} _{-1.39}$ & 17.05$^{+0.12} _{-0.12}$ & 642.55$^{+0.36} _{-0.36}$ & 105.91$^{+1.13} _{-0.97}$ & 163.0 & 2.31 & 5.04 \\
AGC000914$^\ast$$^\star$ & NGC 493 & high S/N & a.100 & 89.06$^{+1.31} _{-1.22}$ & -0.321$^{+0.016} _{-0.017}$ & 21.91$^{+0.68} _{-0.66}$ & 0.897$^{+0.032} _{-0.035}$ & 45.68$^{+7.98} _{-8.4}$ & 27.05$^{+0.28} _{-0.27}$ & 2368.17$^{+1.25} _{-1.35}$ & 204.42$^{+2.76} _{-2.52}$ & 165.2 & 2.69 & 5.07 \\
AGC000942$^\mathsection$ &  & high S/N & a.100 & 13.85$^{+0.58} _{-0.44}$ & -0.075$^{+0.042} _{-0.055}$ & 7.54$^{+0.78} _{-0.71}$ & 0.513$^{+0.201} _{-0.158}$ & 15.62$^{+1.73} _{-0.8}$ & 5.89$^{+0.08} _{-0.08}$ & 2334.88$^{+0.31} _{-0.32}$ & 36.19$^{+0.61} _{-0.56}$ & 99.8 & 2.11 & 2.24 \\
AGC000947$^\ast$$^\ddagger$ & NGC 514 & high S/N & a.100 & 115.03$^{+0.25} _{-0.25}$ & 0.016$^{+0.008} _{-0.008}$ & 11.62$^{+0.34} _{-0.32}$ & 0.765$^{+0.017} _{-0.017}$ & 77.21$^{+3.01} _{-3.19}$ & 25.54$^{+0.18} _{-0.18}$ & 2471.61$^{+0.25} _{-0.26}$ & 241.43$^{+0.66} _{-0.66}$ & 169.2 & 2.29 & 4.4 \\
AGC000957$^\star$$^\mathsection$ & KDG 5 & high S/N & a.100 & 25.17$^{+2.57} _{-1.72}$ & 0.494$^{+0.096} _{-0.124}$ & 17.26$^{+3.03} _{-4.28}$ & 0.56$^{+0.264} _{-0.29}$ & 38.6$^{+18.06} _{-5.81}$ & 10.15$^{+0.18} _{-0.15}$ & 2149.57$^{+4.28} _{-2.82}$ & 74.75$^{+5.83} _{-3.41}$ & 111.0 & 2.19 & 2.4 \\
AGC000966$^\ast$$^\star$$^\ddagger$ & NGC 520 & high S/N & a.100 & 77.68$^{+2.31} _{-1.71}$ & 0.633$^{+0.003} _{-0.009}$ & 24.92$^{+0.06} _{-0.15}$ & 0.555$^{+0.015} _{-0.016}$ & 188.34$^{+7.32} _{-10.62}$ & 30.96$^{+0.44} _{-0.5}$ & 2201.14$^{+1.65} _{-1.97}$ & 244.64$^{+4.89} _{-4.09}$ & 140.0 & 3.02 & 12.9 \\
AGC001102$^\star$$^\ddagger$ & CGCG 412-002a & high S/N & a.100 & 40.99$^{+3.64} _{-3.67}$ & 0.595$^{+0.031} _{-0.054}$ & 23.77$^{+0.93} _{-1.6}$ & 0.803$^{+0.138} _{-0.187}$ & 52.68$^{+14.9} _{-7.4}$ & 9.56$^{+0.16} _{-0.16}$ & 1971.4$^{+3.65} _{-4.49}$ & 110.21$^{+6.8} _{-6.45}$ & 96.1 & 2.13 & 2.3 \\
AGC001133 & M+105005 & high S/N & a.100 & 50.73$^{+0.37} _{-0.41}$ & 0.135$^{+0.012} _{-0.012}$ & 12.61$^{+0.39} _{-0.38}$ & 0.841$^{+0.042} _{-0.045}$ & 25.37$^{+3.64} _{-3.92}$ & 15.2$^{+0.09} _{-0.09}$ & 1964.94$^{+0.28} _{-0.27}$ & 115.48$^{+0.92} _{-1.23}$ & 171.4 & 1.92 & 2.56 \\
AGC001149$^\ast$ & NGC 628 & high S/N & a.100 & 22.37$^{+0.04} _{-0.04}$ & 0.057$^{+0.002} _{-0.002}$ & 8.48$^{+0.05} _{-0.04}$ & 0.383$^{+0.004} _{-0.004}$ & 21.14$^{+0.03} _{-0.03}$ & 421.25$^{+0.21} _{-0.2}$ & 658.21$^{+0.02} _{-0.02}$ & 52.28$^{+0.03} _{-0.03}$ & 2687.5 & 4.62 & 52.52 \\
AGC001175 &  & high S/N & a.100 & 39.46$^{+0.38} _{-0.54}$ & -0.018$^{+0.017} _{-0.017}$ & 9.44$^{+0.62} _{-0.62}$ & 0.665$^{+0.112} _{-0.102}$ & 21.19$^{+3.53} _{-4.53}$ & 14.82$^{+0.14} _{-0.12}$ & 729.17$^{+0.32} _{-0.31}$ & 86.24$^{+2.28} _{-2.67}$ & 142.2 & 2.59 & 3.47 \\
AGC001176$^\star$$^\mathsection$ & DDO 13 & high S/N & a.100 & 15.18$^{+0.31} _{-0.33}$ & -0.277$^{+0.036} _{-0.035}$ & 8.3$^{+0.35} _{-0.29}$ & 0.493$^{+0.09} _{-0.061}$ & 16.12$^{+0.47} _{-0.31}$ & 31.3$^{+0.1} _{-0.1}$ & 629.57$^{+0.11} _{-0.12}$ & 38.67$^{+0.24} _{-0.21}$ & 418.3 & 2.59 & 5.19 \\
AGC001192$^\ddagger$ & NGC 658 & high S/N & a.100 & 140.22$^{+0.47} _{-0.48}$ & -0.027$^{+0.009} _{-0.009}$ & 19.44$^{+0.66} _{-0.64}$ & 0.886$^{+0.028} _{-0.032}$ & 80.74$^{+12.01} _{-13.68}$ & 26.12$^{+0.21} _{-0.22}$ & 2989.65$^{+0.47} _{-0.47}$ & 304.25$^{+1.99} _{-1.76}$ & 138.4 & 2.57 & 3.5 \\
AGC001195$^\star$$^\ddagger$ & CGCG 437-010 & high S/N & a.100 & 57.55$^{+1.17} _{-1.24}$ & 0.537$^{+0.046} _{-0.039}$ & 17.47$^{+0.33} _{-0.35}$ & 0.861$^{+0.034} _{-0.045}$ & 26.18$^{+4.41} _{-3.87}$ & 25.91$^{+0.14} _{-0.14}$ & 779.88$^{+1.12} _{-1.11}$ & 133.78$^{+1.85} _{-1.65}$ & 216.7 & 2.52 & 4.68 \\
\multicolumn{15}{c}{$\cdots$}\\
UGC 7608$^\star$ &  & SPARC & T88 & 23.29$^{+0.92} _{-0.45}$ & -0.249$^{+0.029} _{-0.038}$ & 11.06$^{+0.44} _{-0.51}$ & 0.941$^{+0.043} _{-0.108}$ & 24.79$^{+102.06} _{-8.86}$ & 19.04$^{+0.45} _{-0.26}$ & 533.37$^{+0.5} _{-0.5}$ & 58.99$^{+1.36} _{-0.98}$ & 104.9 & 9.53 & 8.34 \\
IC 3687 & UGC 7866 & SPARC & T88 & 19.26$^{+0.31} _{-0.35}$ & -0.047$^{+0.024} _{-0.025}$ & 5.97$^{+0.56} _{-0.45}$ & 0.393$^{+0.062} _{-0.041}$ & 18.05$^{+0.33} _{-0.31}$ & 14.19$^{+0.08} _{-0.08}$ & 353.27$^{+0.18} _{-0.17}$ & 44.4$^{+0.38} _{-0.32}$ & 222.6 & 4.09 & 5.49 \\
NGC 5289 & UGC 8699 & SPARC & T88 & 174.85$^{+0.68} _{-0.68}$ & 0.013$^{+0.019} _{-0.019}$ & 12.83$^{+0.83} _{-0.72}$ & 0.961$^{+0.03} _{-0.051}$ & 125.48$^{+49.28} _{-82.21}$ & 6.15$^{+0.15} _{-0.15}$ & 2523.84$^{+0.72} _{-0.72}$ & 367.78$^{+2.07} _{-1.97}$ & 51.9 & 1.45 & 1.33 \\
UGC 8837$^\ast$$^\star$ &  & SPARC & T88 & 34.72$^{+0.16} _{-0.17}$ & 0.402$^{+0.007} _{-0.007}$ & 16.43$^{+0.14} _{-0.14}$ & 0.968$^{+0.013} _{-0.014}$ & 145.45$^{+38.02} _{-49.89}$ & 15.46$^{+0.19} _{-0.16}$ & 146.89$^{+0.2} _{-0.2}$ & 89.44$^{+1.07} _{-0.9}$ & 417.4 & 1.55 & 7.66 \\
UGC 9992 &  & SPARC & T88 & 16.79$^{+0.45} _{-0.32}$ & 0.166$^{+0.036} _{-0.027}$ & 6.9$^{+0.53} _{-0.54}$ & 0.665$^{+0.134} _{-0.11}$ & 17.58$^{+1.92} _{-1.08}$ & 6.51$^{+0.06} _{-0.06}$ & 427.95$^{+0.22} _{-0.23}$ & 41.51$^{+0.51} _{-0.49}$ & 157.1 & 3.11 & 3.03 \\
UGC 12632 &  & SPARC & T88 & 48.88$^{+0.07} _{-0.08}$ & -0.077$^{+0.003} _{-0.003}$ & 10.53$^{+0.1} _{-0.11}$ & 0.871$^{+0.014} _{-0.013}$ & 29.35$^{+1.48} _{-1.7}$ & 42.43$^{+0.08} _{-0.09}$ & 421.33$^{+0.07} _{-0.06}$ & 109.99$^{+0.34} _{-0.31}$ & 581.6 & 2.39 & 6.3 \\
Mrk 209$^\dagger$ & UGCA281 & SPARC & T88 & 18.39$^{+4.62} _{-4.09}$ & -0.086$^{+0.142} _{-0.167}$ & 14.15$^{+2.66} _{-2.16}$ & 0.722$^{+0.234} _{-0.388}$ & 18.12$^{+3.76} _{-4.48}$ & 6.23$^{+0.1} _{-0.09}$ & 280.75$^{+1.08} _{-1.61}$ & 49.13$^{+1.94} _{-2.44}$ & 81.0 & 4.4 & 4.4 \\
IC 2574 &  & SPARC & R80 & 44.6$^{+0.11} _{-0.09}$ & 0.102$^{+0.001} _{-0.001}$ & 17.11$^{+0.07} _{-0.07}$ & 0.955$^{+0.003} _{-0.003}$ & 13.86$^{+0.46} _{-0.4}$ & 406.13$^{+0.26} _{-0.25}$ & 57.77$^{+0.04} _{-0.04}$ & 108.91$^{+0.11} _{-0.11}$ & 1875.9 & 14.59 & 27.83 \\
NGC 2403 &  & SPARC & R80 & 108.83$^{+0.02} _{-0.02}$ & -0.08$^{+0.0} _{-0.0}$ & 16.93$^{+0.03} _{-0.03}$ & 0.769$^{+0.001} _{-0.001}$ & 60.64$^{+0.2} _{-0.2}$ & 1435.68$^{+0.43} _{-0.44}$ & 138.76$^{+0.02} _{-0.02}$ & 234.26$^{+0.08} _{-0.08}$ & 3649.1 & 18.56 & 151.63 \\
M 109 & NGC 3992 & SPARC & R80 & 171.78$^{+0.41} _{-0.39}$ & -0.139$^{+0.011} _{-0.01}$ & 12.85$^{+0.41} _{-0.41}$ & 0.999$^{+0.001} _{-0.004}$ & 119.51$^{+55.16} _{-78.19}$ & 38.5$^{+0.4} _{-0.41}$ & 1152.79$^{+0.41} _{-0.4}$ & 361.56$^{+0.96} _{-0.97}$ & 105.3 & 17.08 & 17.91 \\
\hline
\end{tabular}

